Worst-case Delay Analysis of Time-Sensitive Networks with Deficit Round-Robin

In feed-forward time-sensitive networks with Deficit Round-Robin (DRR), worst-case delay bounds were obtained by combining Total Flow Analysis (TFA) with the strict service curve characterization of DRR by Tabatabaee et al. The latter is the best-known single server analysis of DRR, however the former is dominated by Polynomial-size Linear Programming (PLP), which improves the TFA bounds and stability region, but was never applied to DRR networks. We first perform the necessary adaptation of PLP to DRR by computing burstiness bounds per-class and per-output aggregate and by enabling PLP to support non-convex service curves. Second, we extend the methodology to support networks with cyclic dependencies: This raises further dependency loops, as, on one hand, DRR strict service curves rely on traffic characteristics inside the network, which comes as output of the network analysis, and on the other hand, TFA or PLP requires prior knowledge of the DRR service curves. This can be solved by iterative methods, however PLP itself requires making cuts, which imposes other levels of iteration, and it is not clear how to combine them. We propose a generic method, called PLP-DRR, for combining all the iterations sequentially or in parallel. We show that the obtained bounds are always valid even before convergence; furthermore, at convergence, the bounds are the same regardless of how the iterations are combined. This provides the best-known worst-case bounds for time-sensitive networks, with general topology, with DRR. We apply the method to an industrial network, where we find significant improvements compared to the state-of-the-art.

==> algorithm.tex <==
% !TeX root = mainRTSS.tex
TODO

==> computationFixPoint.tex <==
% !TeX root = mainDRR.tex

\section{Computation of \thref{thm:optDrrService}}

\begin{algorithm}[htbp]
	\textbf{Input:}{\\
		Quantum $Q_1, Q_2, \ldots, Q_n$\\
		Maximum Packet size: $\lmax_1, \lmax_2, \ldots, \lmax_n$\\
		Maximum Deficit: $\mdelta_1, \mdelta_2, \ldots, \mdelta_n$\\
		Arrival Curves: $\alpha_1,\alpha_2, \ldots, \alpha_n$
	}
	%\textbf{Data:} {Maximum weight: $w_{\max} = max\{w_1,..,w_n\}$}
	\caption{Interleaved Weighted Round-Robin}
	\begin{algorithmic}[1]
		\State $w_{\max} = \max\{w_1,..,w_n\}$
		\While{True}
		\Comment{A round starts.}
		\For{$C\leftarrow 1$ to $w_{\max}$}
		\Comment{A cycle starts.}
		\For{$i \leftarrow 1 $ to $n$}
		\If{$C \leq w_i$}%\Comment{Queue $i$ is visited.} \label{alg:visit}
		\If{(\textbf{not} empty($i$))}\\
		\Comment{A service for queue $i$.}
		\State \texttt{print}(\text{now},$i$);\label{alg:service}
		\State \texttt{send}(head($i$));
		\State\texttt{removeHead(}$i$);
		\EndIf
		\EndIf
		\EndFor
		\EndFor \Comment{A cycle finishes.}
		\EndWhile \Comment{A round finishes.}
	\end{algorithmic}
	\label{alg:IWRR}
\end{algorithm}


==> method.tex <==
% !TeX root = mainRTSS.tex

\section{Refinement Phase: Shared Memory Parallelization}
\label{sec:refinePhase}

In Section \ref{sec:initPhase}, some valid bounds for $( \beta,d,\zcut ,b)$ are obtained. These bounds are obtained by TFA and we want to improve on them using PLP. Number of refinements exist: PLP can be applied to refine bounds on burstiness everywhere, and hence arrival curves. Then, given improved arrival curves, DRR strict service curves can be improved; given improved arrival curves and service curves, per-node delay bounds can be improved. These improved DRR strict service curves and per-node delay bounds can further improve the bounds obtained by PLP. Hence, we have set of refinements such that the output of each can be fed back to another. Also, they can be applied in any order. The question is how we could get the best out of it, and in what order should we use them. We present this phase using shared memory parallelization \cite{shared_parallel} (see Fig.~\ref{fig:gen_method}): We consider a shared memory that contains $( \beta,d,\zcut ,b)$, and we have number of workers that chooses a refinement, read some values of the shared memory, improve some, and make an update in the shared memory. We show that if each refinement is visited infinite times, the limit shared memory exist and is independent of the order and the time that each refinement is visited.

% We present this phase using shared memory parallelization \cite{shared_parallel} (see Fig.~\ref{fig:gen_method}): We consider a shared memory that contains $( \beta,d,\zcut )$, and we have set of refinements that read some values of the shared memory, improve some, and make an update in the shared memory. We show that if each refinement makes an update infinite times, the shared memory converges to a unique fixed-point, regardless of the order each refinements made an update.



\subsection{Generic Scheme Implementation of the Refinement Phase Using Shared Memory Parallelization} %\label{sec:genMethod}
%\begin{figure*}[htbp]
%	\centering
	% \includegraphics[width=0.75\linewidth]{RTSS2022/TON_v1/Figures/whole_method.pdf}
%	\input{RTSS2022/TON_v1/Figures/method_sketch}
%		\caption{\sffamily \small Overview of the method. We consider a shared memory  that contains $( \beta,d,\zcut )$. It is initialized by the bounds obtained at the initial phase in Section \ref{sec:initPhase} when using TFA. Then, at refinement phase of Section \ref{sec:refinePhase}, number of refinements run in parallel; each read some components of the shared memory and update some. Each refinement is infinite times visited, until the shared memory converges to the fixed point. Then, final values of the shared memory are post-processed in Section \ref{sec:postPhase} and end-to-end delay bounds are obtained for flows of interest.
%	\anne{Questions: 1) are we allowed to change fonts like that? 2) Why not having $PLP^{backlog}$ by itself? It is used twice, so we might compute twice the same  functions to gets delay / DRR curves}
%	}
%	\label{fig:gen_method}
%\end{figure*}

We consider a distributed system where we have a shared memory of $( \beta,d,\zcut ,b)$, number of workers, and a set of refinements. The shared memory is initialized by the bounds obtained in Section \ref{sec:initPhase}. Every worker has read and write access to the shared memory: Whenever a worker is free, it chooses a refinement; it then read some values stored in the shared memory that are needed to apply the refinements. It then computes the refined bounds, and it should wait for the memory to be unlocked (if it is locked at time); then it has an access to memory, and it can make an update and read the values; in this short interval the memory is locked. When updating some values, we take we take the minimum (maximum for service curves) of the value in the shared memory and the computed values of the worker; this is because some values might be already improved by other workers. Each refinement should be infinitely often visited; it means there should be another visit to a refinement after any time.

We will now explain the set of refinements that can be used.


% and waits for the memory to be unlocked. When it gains an access to the memory, the memory is locked for a short period of  time. 

% every worker has read and write access to the shared memory. We have a set of refinements (detailed later) that whenever a worker is free, chooses a refinements; then, read the value of the shared memory, and apply the refinement to refine some. Then, when the computation is done, it writes the improved values in the memory. When writting it takes the best of what is 


% We present this phase using shared memory parallelization \cite{shared_parallel}. We consider a shared memory that contains $( \beta,d,\zcut )$. It is initialized by the bounds obtained at the initial phase in Section \ref{sec:initPhase}. Also, we consider three types of refinements that are explained in detail later. Each of these refinements read some values from the shared memory, then refine some values in the shared memory. When reading some values, we temporary lock the memory and it cannot be read or updated by others. When a refinements finishes its task and wants to make an update, it should wait for the memory to be unlocked (if it is locked at time); then it has an access to memory, and it can make an update and read the values. When updating some values, we take we take the minimum (maximum for service curves) of the value in the shared memory. 


\subsubsection{Refinements of bounds at cuts}\label{sec:cut}
As explained in Section \ref{sec:plp}, PLP requires some artificial cuts to create trees. The initial bounds on the propagated burstiness of flows at cuts $\zcut$ are the ones obtained with TFA. However, PLP can compute better bounds  given per-node strict service curves $\beta_i$ and delay bounds $d_i$.

We consider a module for each class $C_i$. Whenever the module of class $C_i$ is called, it first reads $(\beta_i,d_i)$ from the shared memory. Second, it computes improved bounds on the propagated burstiness at cuts $\zcuti = \plpcut_i ( \beta_i, d_i )$. Third, it updates $\zcuti$ in the shared memory.

It might be the case that the bounds obtained for  $d_i$ in the initial phase are infinite, and hence, at a time that the module is called some or all values are $d_i$ are infinite; in such cases, $\plpcut_i$ still can be applied and might return finite bounds. In this case, $d_i$ eventually gets finite values as by the modules of Section \ref{sec:delay} they get refined. If  $\plpcut_i$  returns infinite bounds for class $C_i$, we write infinity for all components of $\zcuti$ in the shared memory.

\subsubsection{Refinements of Output Burstiness}\label{sec:service}
Consider a node $v$ and a class $C_i$ at node $v$. We use our improvement to PLP of Section \ref{sec:plpBack} to compute aggregate output burstiness for class $C_i$ at the output of node $v$. This is denoted by $b_i^* = \plpb_{v,i}(\beta_i,d_i,\zcuti)$. If we have infinite bounds for $\zcuti$, then $\plpb_{v,i}(\beta_i,d_i,\zcuti)$ returns infinity for this class. 

\subsubsection{Refinements of DRR Strict Service Curves}\label{sec:service}
Consider a node $v$. Recall that function ${\beta^v }' = \drrb_v \lp b^* ,\beta^v \rp$, as explained in Section \ref{sec:drrservice_ndm}, improves already available DRR strict service curves $\beta_v$ given $b^*$ bounds on the output burstiness of each class. Even if $b^*$ has infinite components  $\drrb_v$ still can be applied and the result are always finite.

\subsubsection{Refinements of Input Burstiness}\label{sec:service}
Consider a node $v$, a class $C_i$ at node $v$, and an edge $e \in \textrm{In}_i(v)$. We want to compute a bound on the burstiness of flows of class $C_i$ that are carried by the edge $e$. This bounds can used to compute a delay bound at node $v$. We use our improvement to PLP of Section \ref{sec:plpBack} to compute $b_e = \plpb_{e,i}(\beta_i,d_i,\zcuti)$. If we have infinite bounds for $\zcuti$, then $\plpb_{v,i}(\beta_i,d_i,\zcuti)$ returns infinity for this class.


%DRR strict service curves of the initial phase are obtained from the arrival curves that TFA computed. Here, We use PLP and improve  arrival curves at a node and hence the DRR strict service curves. Recall that function ${\beta^v }' = \drrb_v \lp b^* ,\beta^v \rp$, as explained in Section \ref{sec:drrservice_ndm}, improves already available DRR strict service curves $\beta_v$ given $b^*$ bounds on the output burstiness of each class.
%We use our improvement to PLP of Section \ref{sec:plpBack} to compute aggregate output burstiness for every class at the output of node $v$. This is denoted by $b_i^* = \plpb_{v,i}(\beta_i,d_i,\zcuti)$.

% Then, we want to improve these output burstiness using PLP, and hence DRR strict service curves. However, PLP can compute an output burstiness for an individual flow; then to compute an output burstiness  for an aggregate of flows of a class, we need to aggregate the obtained output burstiness  for each flow. This might be pessimistic as we implicitly assume that the worst-case scenario for each flow can be achieved at the same time. This can be improved by using PLP and directly compute an output burstiness for an aggregate of some flows. We provide a minor improvement to PLP. The details and the proof are given in Section \ref{sec:plpBack}. We denote it by $\plpb_{e,i}$ that compute a bound on the burstiness for the aggregate of all flows of class $C_i$ carried by an edge $e$. 


% \begin{theorem}
%     Consider a PLP used to compute backlog bound for a single flow, and a set of flows of interest. Change the objective the PLP to maximize the aggregate backlog bound for a
% % \end{theorem}

% We provide a minor improvement to PLP: We show that  the same PLP used to compute a backlog bound for a single flow can be used yet with one difference: The objective is to maximize the aggregate backlog bound for the flows of interest. The proof is given in Section \ref{sec:proof}. We denote it by $\plpb_{E,i}$ that compute a bound on the burstiness for the aggregate of all flows of class $C_i$ carried by edges in $E$. 

% We consider a refine for every node $v$.  Whenever the module of node $v$ it is called, it first reads $(\beta,d,\zcut)$ from the shared memory.
% Second, it creates some local variables $b_i^*$ for the aggregate output burst of class $C_i$; this variable gets $b_i^* = \plpb_{\scriptsize\textrm{Out}(v),i}(\beta_i,d_i,\zcuti)$. Third, given $b^*$, DRR strict service curve are improved by $\beta^v = \drrb_v \lp b^* ,\beta^v \rp$. Lastly, it updates $\beta^v$ in the shared memory. 

% If when we read values of the shared memory, we have infinite bounds for $\zcuti$ for class $C_i$, then $\plpb_{\scriptsize\textrm{Out}(v),i}$ returns infinity for this class. However, $\drrb_v$ still can be applied and the result are always finite.

\subsubsection{Refinements of Per-node Delay Bounds}\label{sec:delay}
Per-node delay bounds can be improved because of two reasons: First, DRR strict service curves are being refined. Second, PLP can be used to improve the arrival curves. 

Consider a node $v$ and a class $C_i$ at node $v$. To compute a delay bound at node $v$, we want to know the arrival curves of each input ports of node $v$. Because, if a collection of flows arrive on the same link, the rate limitation imposed by the link can be used to improve the arrival curve, for the aggregate. This is known as line-shaping  \cite{Ahlem-line-shaping,Grieu-line-shaping, bouillard2020tradeoff}. Then, we can take into account the effect of line shaping as in Section VI-B of \cite{ludo_cycle}. Let $d^v_i = \mathcal{D}_{v,i}(  b_i ,\beta^v_i)$ be the operation that given $b_i$, a collection of burstiness at each input port of node $v$, and the service curve offered by node $v$ computes a delay bound by taking into account the effect of shaping and packetizer. If $ b_i$ has infinite components, then we $\mathcal{D}_{v,i}(  b_i ,\beta^v_i)$ returns infinity.

  





\subsection{Convergence and Uniqueness}
\begin{theorem}[Correctness and Convergence of PLP Refinement Phase of Section \ref{sec:genMethod}] \label{thm:genMethod}
 Consider a networks with DRR scheduling per class, as described in Section \ref{sec:sysmodel}. Assume $\lp \beta,d,\zcut \rp $, valid  per-node and  per-class DRR strict service curves,  per-node and per-class delay bounds, and per-class propagated burstiness at cuts. Consider the generic method of Section \ref{sec:genMethod} where the shared memory  is initialized   with $\lp \beta,d,\zcut \rp $. Let $\lp \beta',d',{\zcut}' \rp $ be the values of the shared memory at a time after initialization. Then,
 \begin{enumerate}
    \item $\lp \beta',d',{\zcut}' \rp$ is valid.
    \item $\lp \beta',d',{\zcut}' \rp$ converges to a fixed-point, provided that each refinements is applied infinite times.
    \item The fixed point is unique and  regardless of the order each refinement is visited, given initial bounds $\lp \beta',d',{\zcut}' \rp $
 \end{enumerate}
\end{theorem}

The proof is in Section \ref{sec:proof}. We now present two implementations of the method, where we explain in what order we can apply the refinements. By Theorem \ref{thm:genMethod}, we know the order does not effect the final result, however, in our implementations we 


\subsection{Two Implementations of PLP Refinements}
\begin{figure*}[htbp]
	\centering
	%  \title={.}
	\begin{subfigure}[b]{0.85\textwidth}
		\centering
		% include first image
		\includegraphics[width=\linewidth]{TON_v1/Figures/v1_para.pdf}
		\caption{	Version 1 	}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.85\textwidth}
		\centering
		% include first image
		\includegraphics[width=\linewidth]{TON_v1/Figures/v2_para.pdf}
	\caption{	Version 2 	}
	\end{subfigure}
	\caption{\sffamily \small Two suggested order to apply each refinement. In both version, first bounds on the burstiness of flows at cuts $\zcut$ are updated; then, each node is visited with respect to the topological order of the tree; DRR strict service curve and then delay bounds are updated. For version 2, at each node we iterate until the delay bounds converge. We then start over and update $\zcut$.}
	\label{fig:versions}
\end{figure*}

We presented the generic presentation of this phase. By Theorem \ref{thm:genMethod}, any implementation results in the same final bounds. TIn this section, we present two versions of implementations where we believe are more time-efficient.
% Assume we have $W$, with $W \geq 1$ workers that can run in parallel. In this section, we create a list of task that fixes the order that each refinements should be visited; then, a free worker run  the first undone task in the list.

\subsubsection{Version 1}
This version is illustrated in Fig.~\ref{fig:v1}. We first, refine the bounds on the burstiness at cuts for every class. This is because if for a class might be considered unstable in the initial phase, i.e., obtained bounds are infinite. As PLP gives a larger stability region compared to TFA, bounds on burstiness of flows at cuts might become finite at this point. Then, PLP method to obtain backlog bound used in other refinements also provides finite bounds. Hence, we give a priority to $\plpcut$ refinements. If we have multiple workers, these tasks can be run in parallel. We then go through each node $v$; at each node $v$ we can use the refinements of DRR strict service curves and delay bounds; we apply the later for every class $C_i$ at node $v$. The computation of each node can be parallelized.
% The list of task 1 is illustrated in \ref{fig:versions}. We first update $\zcut_i$ for each class $i$. We then sort nodes $v$ in topological order; then, at each node $v$, the service curves and then the delay bounds are updated. When, every node $v$ was visited, we start over.

\subsubsection{Version 2}
Version 2 has one difference compared to Version 1 (see Fig.~\ref{fig:v2}): When we visit a node, we use two refinements. One for s

% Depending on the network topology, $\plpcut$ can be very costy. Hence, we modify Version 1 such that $\plpcut$ runs when other refinements are exhausted. Specifically, when a node is visited, we iterate between  DRR strict service curve refinements and delay bounds until the delay bounds converges. See \ref{fig:versions}.

% The output burstiness of class $C_i$ at node $v$ is equal to the aggregate output burstiness of all flows of class $C_i$   that exits $v$.
% PLP, as is, can compute  a bound on the propagated burstiness for an individual flow; then to compute a  a bound for the aggregate of the propagated burstiness of some flows, we need to aggregate the obtained bound for each flow. This might be pessimistic as it is implicitly assumed that the worst-case scenario to maximize the burstiness for each flow can be achieved at the same time. To mitigate this, we provide a minor improvement to PLP such that it directly computes a bound on the burstiness for an aggregate of some flows. We denote it by $\plpcut$




% We first present a generic method, and give some theoretical result about it; our generic method is an arbitrary use of our bag of refinements.  Then, we give two versions of its implementations.


% Our method can be divided into three main phases:
% \begin{itemize}
%     \item \textbf{Phase 0:} Compute some valid $\lp \beta,d,z \rp $ (i.e., per-node DRR strict service curves,  per-node delay bounds, and propagated burstiness), using existing method, i.e., Algorithm \ref{alg:tfa} in Section \ref{sec:tfa}.
%     \item \textbf{Phase 1:} Improve $\lp \beta,d,z \rp $, as much as possible, by means of refinements of Table \ref{tab:cat}, in an iterative way.
%     \item \textbf{Phase 2:} Given the improved $\lp \beta,d,z \rp $, use iPLP and compute an end-to-end delay bound for the flows of interest.
% \end{itemize}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[htbp]
% \centering
% \caption{Catalog of Refinements of Phase 1}
% \label{tab:cat}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l}
% $d_i^v = \mathcal{D}_{v,i}^{\scriptsize\textrm{NC}}\lp  z_i^{\textrm{In}(v)} ,\beta^v_i\rp $ & Network calculus delay bound  for class $C_i$ at node $v$.            \\ \hline
% ${\beta^v}' = \drrb_v \lp z^{\textrm{Out}(v)} ,\beta^v \rp$                              & Refines a collection of strict service curves  $\beta(v)$ at node $v$. \\ \hline
% $z_i^{E^{\scriptsize\textrm{cut}}_i} = \plpcut_i \lp \beta_i, d_i\rp $ &
%   Upper bounds the burstiness of flows of class $C_i$ at cuts $E^{\scriptsize\textrm{cut}}_i$. \\ \hline
% $z_i^{\textrm{Out}(v)}  = \plpb_{v,i} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$. &
%   Upper bounds the burstiness of class $C_i$ at the output of node $v$.
% \end{tabular}%
% }
% \end{table*}

% Phase 0 and Phase 1 are clear, and the non-trivial part of the method is Phase 1. Let us elaborate on it. The refinements we use in this phase is summarized at Table~\ref{tab:cat}: The first two are node analysis (i.e., given burstiness and strict service curves at node $v$, refine per-node delay or strict service curve at that node). The second two refinements are network analysis (i.e., given per-node delay bounds and strict service curves of all nodes, and bounds on burstiness of  flows at cuts, improve the some bounds on the burstiness). 

% The essence of the refinements are as follows: Each of these refinements takes as input $\lp \beta,d,z \rp $ (i.e., Per-node DRR strict service curves,  Per-node delay bounds, and Propagated burstiness), and improves them, i.e, it outputs $\lp \beta',d',z' \rp $, where $\beta' \geq \beta$, $d' \leq d$, and $z' \leq z$. Then,  $\lp \beta',d',z' \rp $ can be fed back to another or the same refinement. The method is summarized in Fig.~\ref{fig:gen_method}.

% The question is how we could get the best out of it. In what order should we use them? How many times should we apply each?  Is there a fixed-point or the final result depends on how we combine these operations? We answer all in the following theorem.


\section{Post-process Phase: iPLP for End-to-end delay bounds} \label{sec:postPhase}
  When the refinement phase of Section \ref{sec:refinePhase} is converged, we proceed and compute end-to-end delay bound for each flow of interest. Strict service curves $\beta$ obtained are piece-wise linear and convex. Buy, they can be improved by taking into account the non-convex strict service curve of Fig.~\ref{fig:ncService}. However,  PLP only supports   piece-wise linear and convex service curves. We introduce two binary variables at each node  to support non-convex service curves such as Fig.~\ref{fig:ncService}; we call this new PLP, iPLP.

 
  
%   We first present the linear program that PLP solves. We then explain what constraints we add to it to build iPLP. PLP considers an arrival and a departure time of a bit of interest; it then extracts number of times at each node. These times are represented by a variable inside PLP. For each time variable at a node, the number of bits observed at each time variable for each flow is represented by a variable. Then, some linear constraints are obtained by writing network calculus relations such as arrival curve constraints at sources for all flows, service curve constraints at all nodes, and etc. as linear constraints; then, a linear program maximize delay or backlog of the bit of interest. To construct iPLP, we use the exact same PLP but we add some new constraints to the service curve constraints. In this paper, we only present the service curve constraints of PLP, and the details can be found in Section 4 of \cite{plp}. We map our notation to the ones used in \cite{plp} to enable an interested reader tp completely implement iPLP. 
  
%   Consider per-class network of class $C_i$: The last server traversed by the flow of interest becomes the root of the tree. As we assume  a tree, it follows that each node $v$, except the root, has a unique successor. We denote the successor of node $v$ by $\suc(v)$, and we add an artificial node to be the successor of the root. Define $\depth$ as follows: Let $\depth(\pi_{\bar{f}}(l_{\bar{f}})+1) = 1$ and for every $n$, $\depth(v) = \depth\lp \suc\lp v \rp  \rp + 1$. 
  
%   Time Variables: For every node $v$, define  $\tvar{v}{k}$ with $k \in \{1, \ldots, \depth(v) \}$. It can be mapped to $\mathbf{t}_{(n,k)}$ of \cite{plp} by mapping $n$ to $v$.
  
  
%   Process Variables: For every node $v$ and every $g$ at $v$, define $\fvar{v}{f}{v}{k}$ with $k \in \{1, \ldots, \depth(v) \}$, where  $\fvar{v}{f}{v}{k}$ is a variable for the cumulative arrival function of flow $f$ at the input of node $v$ at time $\tvar{v}{k}$.  It can be mapped to $\mathbf{F}^j_i\mathbf{t}_{(j,k)}$ of  \cite{plp} by mapping $j$ to $v$, $i$ to $f$.
  
   

   
%   For each flow $f$, let $\pi_f$ be the path of flow $f$, a sequence of nodes that $f$ traverse. Assume that this path has length $l_f$, and thus, $\pi_f(1)$  and $\pi_f(l_f)$ denote the first and last server, respectively, traversed by $f$. 
%   PLP considers a bit of interest of the flow of interest $\bar{f}$ and  it defines two variables for this bit of interest: The time that it arrives at and departures the system. Node $\pi_{\bar{f}}(l_{\bar{f}})$ is the root of the tree.  As we assume  a tree, it follows that each node $v$, except the root $\pi_{\bar{f}}(l_{\bar{f}})$, has a unique successor. We denote the successor of node $v$ by $\suc(v)$, and we let $\suc(\pi_{\bar{f}}(l_{\bar{f}})) = \pi_{\bar{f}}(l_{\bar{f}}) + 1$. Define $\depth$ as follows: Let $\depth(\pi_{\bar{f}}(l_{\bar{f}})+1) = 1$ and for every $n$, $\depth(v) = \depth\lp \suc\lp v \rp  \rp + 1$.





% Time: $\forall$ node $v$, let $u = \suc(v)$\\
% 1) $\forall k \in \{1,\ldots,\depth(v)-1\}, \tvar{v}{k} \geq \tvar{v}{k+1}$\\
% 2) $\forall k \in \{1,\ldots,\depth(v)\}, \tvar{u}{k} \geq \tvar{v}{k}$

        
% FIFO: $\forall$ node $v$ and $\forall k \in \{1,\ldots,\depth(u) \}$, let $u = \suc(v)$\\
% $\forall g \in \textrm{In}(v).~\fvar{v}{g}{v}{k} == \fvar{u}{g}{u}{k}$

% Service: $\forall$ node $n$,\\
% 1) $\sum_{g \in \textrm{In}(v)}\lp \fvar{u}{g}{u}{\depth(u)} - \fvar{v}{g}{v}{\depth(v)} \rp \geq 0$\\
% 2) $\sum_{g \in \textrm{In}(v)}\lp \fvar{u}{g}{u}{\depth(u)} - \fvar{v}{g}{v}{\depth(v)} \rp \geq R^v_i\lp \tvar{u}{\depth(u)} - \tvar{v}{\depth(v)} - T^v_i \rp $\\

% TFA: $\forall$ node $v$ and $\forall k \in \{1,\ldots,\depth(u) \}$,\\
% $\tvar{u }{k} - \tvar{v}{k} \leq d^v_i$

% Arrivals:  $\forall$ flow $f$, 
% $\forall k < k' \in \{1,\ldots,\depth(\pi_{f}(1))\},~\fvar{\pi_{f}(1)}{k'}{f}- \fvar{\pi_{f}(1)}{k}{f} \leq b_f + r_f \lp\tvar{\pi_{f}(1)}{k'} -  \tvar{\pi_{f}(1)}{k}\rp $

   
% Shaping:$\forall$ node $n$,  let $F^* = \textrm{flows}(n) \cap \textrm{flows}(\suc(n))$,
%  \item $\forall k < k' \in \{1,\ldots,\depth(n)\}$, $\sum_{f \in F^* } \lp \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{k} - \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{k'}  \rp\leq \lmax + C_n\lp \tvar{\scriptsize\suc(n)}{k}  - \tvar{\scriptsize\suc(n)}{k'} \rp  $
   
        
%     \item Monotonicity: $\forall$ flow $f$, let $n^{*}_f$ be the first node foe $f$, ,
%         \begin{enumerate}
%             \item $\forall k \in \{1,\ldots,\depth(n^{*}_f)-1\}, \fvar{n^{*}_f}{f}{n^{*}_f}{k} \geq \fvar{n^{*}_f}{f}{n^{*}_f}{k+1}  $
%         \end{enumerate}    
        
%     \item Backlog: $\forall k  \in \{1,\ldots,\depth(n^*)\}$,
%       $ \fvar{n^{*}}{\scriptsize\texttt{foi}}{N+1}{1} -  \fvar{n^{*}}{\scriptsize\texttt{foi}}{n^{*}}{k} \leq b_{\scriptsize\texttt{foi}} + r_{\scriptsize\texttt{foi}} \lp \tvar{N+1}{1} - \tvar{n^{*}}{k}   \rp $
        
% \end{enumerate} 




%   then,  it consists of writing network calculus relations such as arrival curve constraints at sources for all flows, service curve constraints at all nodes, and etc. as linear constraints; then, a linear program maximize delay or backlog of the bit of interest. Every possible trajectory scenarios in the network is a feasible solution of PLP, as it satisfies the constraints; hence, the objective is an upper bound on worst-cases in the network. PLP requires a network to be a tree, otherwise some artificial cuts are introduced; PLP then can compute upper bounds on the burstiness of flows at cuts, propagated burstiness at an intermediate node, and end-to-end delay bounds for flows.  
  
  
  
  
%   Consider a node $v$ that offers $\beta^v$ a service curve that has two parts; a piece-wise linear convex and non-convex part, i.e., $\beta^v = \max \lp\beta^{\scriptsize\textrm{c},v},\beta^{\scriptsize\textrm{nc},v} \rp $; consider $\beta^{\scriptsize\textrm{nc},v}$ as shown in Fig.~\ref{fig:ncService}.  Construct iPLP  as follows: Define all variables and write all constraints exactly as PLP for delay bounds yet with one difference: At each node $v$, define $b_v \in \{0,1\}$ and add the following constraints:
% \begin{align}
%      D(t) - A(s) &\geq 0\\\label{eq:nc1}
%      D(t) - A(s) &\geq c_v(t-T_1) - Mb_v\\
%      D(t) - A(s) &\geq c_v(T_2-T_1) - M(1-b_v)\\
%      t - s &\leq T_2 + Mb_v\\
%      t - s &\geq T_2 - M(1-b_v)\label{eq:nc4}
% \end{align}
% where $M$ is a large positive integer.



% \subsection{Implementations of Our Generic Method}
% Implementations of Phase 0 and 2 are as described. However, Phase 1 can be implemented in infinite ways. We here present two versions of such implementations that we think are the best ones in sense of time and computation complexity. These two are summarized in Algorithm \ref{alg:phase1} and Fig.~\ref{fig:phase1}.

% Version 1 is applying each refinement in series: First, the burstiness of flows at cuts is updated by PLP. Then, at each node i the topological order of the tree, the out put burstiness is obtained by PLP; then, it is used to update DRR service curve and hence the per-node delay bound. However, as $\plpcut$ might be costly \cite{PLP}, we presented version 2; the difference of version two is to visit $\plpcut$ less, and only we exhaust all other refinements. How much costly $\plpcut$ is depends on the network topology and  the number of the cut flows.

% \begin{algorithm}[htbp]
% 	\caption{Phase 1 - Version 1 and 2}
% 	\textbf{Input: }{$\forall \textrm{class } C_i:$\\
% 	$\beta_i$: valid strict service curves at all nodes.\\
% 	$ d_i$: valid delay bounds at all nodes.
% 	}\\

		
% 	\begin{algorithmic}[1]
%     \While{$z$ is not converged}
%     	\For {each class $C_i$ }
% 	        \State $z_i^{E^{\scriptsize\textrm{cut}}_i} \gets \plpcut_i \lp \beta_i, d_i\rp  $
%     	\EndFor\\
	
%         \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$} \Comment{in topological order}
%             \While{$z^{\textrm{Out}(v)}$ is not converged} \Comment{remove while for Version 1}
% 	    	\For {each class $C_i$ at node $v$ }
% 			    \State  $z_i^{\textrm{Out}(v)}  \gets \plpb_{v} \lp             z_i^{E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$
% 	    	\EndFor\\
		
% 	    	\State  $\beta(v) \gets \drrb_v \lp z^{\textrm{Out}(v)},\beta^v\rp$\\
% 	    	\For {each class $C_i$ at node $v$ }
% 	        	\State  $d_i^v = \mathcal{D}_v^{\scriptsize\textrm{NC}}\lp      z_i^{\textrm{In}(v)} ,\beta^v_i\rp $
% 	        \EndFor
% 	        \EndWhile
% 	    \EndFor\\
% 	 \EndWhile

	
	
% 	\end{algorithmic}
	
	
% 	\textbf{\\Output: }{$\lp d ,\beta, z^{E^{\scriptsize\textrm{cut}}}\rp$: Per-node strict service curve, per-node delay bounds, and bounds on propagated burstiness of flows at cuts}
% 	\label{alg:phase1}
	
% \end{algorithm}
% \begin{algorithm}[htbp]
%     \SetKwInOut{Input}{Input}
% 	\SetKwInOut{Output}{Output}
	
% 	\Input{$ \forall$ class $C_i$: \\
% 	$\beta_i$: valid strict service curves at all nodes.\\
% 	$d_i$: valid delay bounds at all nodes.}
	
% 	\BlankLine
	
% % 	\textbf{Input: }{$\forall \textrm{class } C_i:$\\
% % 	$\beta_i$: valid strict service curves at all nodes.\\
% % 	$ d_i$: valid delay bounds at all nodes.
% % 	}\\

%     \While{$z$ is not converged}{
%     	\For {each class $C_i$ }{
% 	         $z_i^{E^{\scriptsize\textrm{cut}}_i} \gets \plpcut_i \lp \beta_i, d_i\rp  $\;
%     	}
% 	    \BlankLine
%         \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$}{
%         % \Comment{in topological order}
%               \tcp*{\small remove while for version 2}
%             \While{$z^{\textrm{Out}(v)}$ is not converged}{
% 	    	\For {each class $C_i$ at node $v$ }{
% 			      $z_i^{\textrm{Out}(v)}  \gets \plpb_{v} \lp             z_i^{E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$\;
% 	    	}
% 		     \BlankLine
% 	    	$\beta(v) \gets \drrb_v \lp z^{\textrm{Out}(v)},\beta^v\rp$ \;
% 	    	\For {each class $C_i$ at node $v$ }{
% 	        	  $d_i^v = \mathcal{D}_v^{\scriptsize\textrm{NC}}\lp      z_i^{\textrm{In}(v)} ,\beta^v_i\rp $ \;
% 	        }
% 	        }
% }
% 	 }

	
	
	
% 	\Output{$\lp d ,\beta, z^{E^{\scriptsize\textrm{cut}}}\rp$: Per-node strict service curve, per-node delay bounds, and bounds on propagated burstiness of flows at cuts}
% % 	\textbf{\\Output: }{$\lp d ,\beta, z^{E^{\scriptsize\textrm{cut}}}\rp$: Per-node strict service curve, per-node delay bounds, and bounds on propagated burstiness of flows at cuts}
% 	\caption{Phase 1 - Version 1 and 2}
% 	\label{alg:phase1}
	
% \end{algorithm}


% \subsection{iPLP: A PLP That Supports Non-convex Strict Service Curves}

% Note that no matter how we combine them, we have a valid, improved results. This is because we start from valid result of Phase 0, and  all of these operations are refinements (i.e., improve on valid results). Hence, no matter how we combine them, we have a valid, improved result. The question is how we could get the best out of it. The question is in what order we should use them? How many times should we apply each? In what order? Is there a fixed-point or the final result depends on how we combine these operations? 

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[htbp]
% \centering
% \caption{Catalog of Refinements of Phase 1}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l}
% $d_i^v = \mathcal{D}_v^{\scriptsize\textrm{NC}}\lp  z_i^{\textrm{In}(v)} ,\beta^v_i\rp $ &
%   \begin{tabular}[c]{@{}l@{}}Computes a network calculus delay bound  for class $C_i$ at node $v$, \\  given strict service curves $\beta_i^v$ and\\  bounds on the input burliness $z_i^{\textrm{In}(v)}$\end{tabular} \\ \hline
% $z_i^{E^{\scriptsize\textrm{cut}}_i} = \plpcut_i \lp \beta_i, d_i\rp $ &
%   \begin{tabular}[c]{@{}l@{}}Computes  upper bounds on the burstiness of flows of class $C_i$\\   at cuts $E^{\scriptsize\textrm{cut}}_i$ using PLP, \\ given strict service curves $\beta_i$ and \\ delay bounds $d_i$ of all nodes.\end{tabular} \\ \hline
% $z_i^{\textrm{Out}(v)}  = \plpb_{v} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$ &
%   \begin{tabular}[c]{@{}l@{}}Compute a backlog bound for flows of class $i$ at the output of node $v$,  \\ using PLP given strict service curves $\beta_i$ and \\ delay bounds $d_i$ of all nodes, and  \\ bounds on the burstiness of flows at cuts $z_i^ {E^{\scriptsize\textrm{cut}}_i}$\end{tabular} \\ \hline
% ${\beta^v}' = \drrb_v \lp z^{\textrm{Out}(v)} ,\beta^v \rp$ &
%   \begin{tabular}[c]{@{}l@{}}At node $v$, it refines a collection of strict service curves  $\beta(v)$\\  given a collection of upper bounds on the output bursts $ z^{\textrm{Out}(v)} $ \\ using Corollary \textbackslash{}ref\{cor:serviceBurst\}.\end{tabular}
% \end{tabular}%
% }
% \end{table*}






% \subsection{Remark on Degraded Operational Mode} \label{sec:degraded_method}
% % \begin{figure*}[htbp]
% % 	\centering
% % 	\includegraphics[width=0.75\linewidth]{RTSS2022/TON_v1/Figures/method_d_complete.pdf}
% % 	\caption{\sffamily \small Summary of Section \ref{sec:degraded_method}, For Degraded Mode, i.e., no assumption on the interfering traffic.}
% % 	\label{fig:degraded_method}
% % \end{figure*}
% The method presented earlier is for the non-degraded opertional mode, i.e., when flows of interfering classes behaves as expected and some arrival curves can be assumed for them. However, sometimes there is an interest in valid delay bounds of degraded operational mode for some flows of a class of interest,  when the interfering traffic behaves as unexpected. Specifically, no arrival curve can be assumed  for flows of other classes. In such cases, the service curves of the class of interest is independent of the interfering traffic. 

% As in this case, class of interest is isolated from other flows, we only focus $\mathcal{G}_i$,  The graph induced by flows of the class of interest $C_i$. We use Theorem \ref{thm:drrService} to find DRR strict service curves at each output port for class $i$.  Thus, for  class $C_i$, we have a FIFO graph induced by flows, $\mathcal{G}_i$, where nodes have convex piece-wise linear strict service curves and flows have concave arrival curves. Therefore, this case is a direct application of \cite{plp},  and we proceed exactly as \cite{plp} to find end-to-end delay bounds for the flows of interest, yet with one difference: We use iPLP to compute end-to-end delay bounds. 
% % This is summarized in Fig.~\ref{fig:degraded_method}.



% \subsection{Remark on Using PLP instead of TFA only for end-to-end delay bound} \label{sec:trivial}
%  By applying the existing method, as explained in Section \ref{sec:tfa}, per-node delay bounds $d_i$, per-node strict service curves $\beta_i$, and propagated burstiness, including at cuts $z_i^ {E^{\scriptsize\textrm{cut}}_i}$, of all flows of each class $C_i$ is obtained. Thus, we can use PLP to obtain end-to-end delay bounds for a flow of interest $f$: $\dend_f = \plpd_{f} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$; hence, $\dend_f$ is improved compared to the bound obtained by TFA, i.e.,  sum of all per-node delay bounds $d_i$ in the path of flow $f$.
 
%  This is what we call trivial \anne{direct} use of PLP: Given node analysis at every node, PLP can be used to obtain end-to-end delay bounds. However, we show that we can benefit more from PLP rather than this trivial use.  Specifically, in our novel method, we use the network analysis of PLP as a feedback to our node analysis of DRR (i.e., DRR strict service curves), and we iterate; thus, we combine PLP and DRR strict service curve refinements, in an iterative way, to improve node analysis and burstiness of flows at cuts.























% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=0.75\linewidth]{RTSS2022/TON_v1/Figures/v12.pdf}
% 	\caption{\sffamily \small Summary of Section \ref{sec:non_degraded_method}, For Non-Degraded Mode, i.e., some arrival curve can be assumed for the interfering traffic.}
% 	\label{fig:TL}
% \end{figure*}

% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=0.75\linewidth]{RTSS2022/TON_v1/Figures/v2.pdf}
% 	\caption{\sffamily \small Summary of Section \ref{sec:non_degraded_method}, For Non-Degraded Mode, i.e., some arrival curve can be assumed for the interfering traffic.}
% 	\label{fig:v1}
% \end{figure*}
% \begin{figure*}[htbp]
% 	\centering
% 	\includegraphics[width=0.75\linewidth]{RTSS2022/TON_v1/Figures/v1.pdf}
% 	\caption{\sffamily \small Summary of Section \ref{sec:non_degraded_method}, For Non-Degraded Mode, i.e., some arrival curve can be assumed for the interfering traffic.}
% 	\label{fig:v2}
% \end{figure*}




% \subsection{\anne{Convergence and validity (dirty draft)}}

% There are three types of variables on which the Functions act: 
% \begin{itemize}
%     \item The arrival curves
%     \item the DRR service curves for each server and each class
%     \item the TFA++ delays
% \end{itemize}

% There are two main functions that are iterated, and for which the variables are modified: 
% \begin{itemize}
%     \item ${\tt PLP}$: computes new arrival curves at the cuts. The function depends on the arrival curves at the cuts, the residual service curves for each class and the TFA++ delays.
%     \item ${\tt DRR}_j$: computes a new service curve for server $j$ (for each DRR class), using the previous service curves for this server, the output arrival curves from this server. It also updates the TFA++ delay. 
% \end{itemize}
% We assume that these functions take as parameters all the variables (even if they do not depend on them all) and output one value per parameter:
% ${\tt PLP},~{\tt DRR}_j: \mathcal{F}^N \times \mathbb{R}_+^M \to \mathcal{F}^N \times \mathbb{R}_+^M $ (with $N$ and $M$ to be more precisely defined)
% \paragraph{Properties of the functions}
% Let $\beta, \beta'$ represent the DRR service curves at all servers and for all classes, $\alpha, \alpha'$ represent arrival curves for all flows at at all points and $d, d'$ the TFA delays for all servers fo all classes. 

% If $\beta \geq \beta'$, $\alpha \leq \alpha'$ and $d \leq d'$, ${\tt PLP}(\alpha, \beta, d) \leq {\tt PLP}(\alpha', \beta', d')$ and ${\tt DRR}_j(\alpha, \beta, d) \leq {\tt DRR}_j(\alpha', \beta', d')$. 



% Moreover, with no loss of generality, one can always consider that if ${\tt PLP}(\alpha, \beta, d)  = (\alpha', \beta' , d')$, then $\alpha' \leq \alpha$, $\beta'\geq \beta$ and $d'\leq d$ (if needed, it is possible to take  $\alpha'\land '\alpha$ instead of $\alpha'$).

% If $\beta \geq \beta'$, $\alpha \leq \alpha'$ and $d \leq d'$, we write $\chi = (\alpha, \beta, d) \leq (\alpha', \beta', d') = \chi'$, so we can write that 
% \begin{itemize}
%     \item ${\tt PLP}(\chi) \leq \chi$ (and similarly for ${\tt DRR}_j$);
%     \item $\chi \leq \chi' \implies {\tt PLP}(\chi) \leq {\tt PLP}(\chi')$ (and similarly for ${\tt DRR}_j$).
% \end{itemize}


% \paragraph{Convergence}
% Consider an infinite sequence $h_1, \ldots, h_n, \ldots$ of functions that are either ${\tt PLP}$ or ${\tt DRR}_j$, and for a given $\chi_0$, compute $\chi_n = h_{n}(\chi_{n-1})$. This results in three sequences $(\alpha_n)_n$, $(\beta_n)_n$ and $(d_n)_n$ that are respectively non-increasing, non-decreasing and non-increasing. 

% \begin{itemize}
%     \item for each flow $f$ and each server $s$, $\alpha_{f, s}$ (arrival curve of flow $f$ at server $s$) is token-bucket, and its arrival rate is always equal to the arrival rate of that flow. So only the burst is modified, cannot increase. As it is positive, it converges. 
%     \item Similar for the delays: for each class and each server, $(d_n^{s, c})_n$ is non-increasing and in $\mathbb{R}_+$, so it converges. 
%     \item From Theorem 2, the service curves for each class and each server are piecewise linear convex, and can only have slopes in a predefined finite set. As a consequence, $\beta_n^{s, c}$ can be written as the maximum of rate-latency curves with predefined slopes, and the latency corresponding to each slope cannot increase. Then they can only converge. 
% \end{itemize}

% \paragraph{Convergence to a unique value (fixed point)}
% Now consider two sequences $(h_n)$and $(h'_n)$ that contain an infinite number of occurrence of each function. Then if $\chi_0 = \chi'_0$, then $(\chi_n)$ and $(\chi'_n)$ converge to the same value (with obvious notations). 

% Because there is an infinite number of occurrences of each function, there exists an increasing sequence $\phi$ such that for all $n\in\mathbb{N}$, $h_n = h'_{\phi(n)}$. 
% For all $n\in\N$, $\chi'_{\phi(n)} \leq \chi_n$. 
% First, this is true by assumption for $n=0$. Suppose this is true for $n-1$. Then we have $\chi'_{\phi(n) - 1} \leq \cdots \leq \chi'_{\phi(n-1)} \leq \chi_{n-1}$, and as $h_n = h'_{\phi(n)}$, we have $\chi'_{\phi(n)} = h_n(\chi'_{\phi(n) - 1}) \leq h_n(\chi_{n-1}) = \chi_n$, and this is true for $n$, which shows by induction, that $\lim_{n\to\infty} \chi'_n \leq \lim_{n\to\infty} \chi_n$. Inverting the roles of $(h_n)$ and $(h'_n)$ enables to conclude that the limits are in fact the same. 

% \jylb{If I understand well this applies to any finite set $\calF$ of isotone mappings $(\Reals^+)^I \to (\Reals^+)^I $ such that $f(z)\leq z$ for all $z\in (\Reals^+)^I$ and all $f\in\calF$: for a sequence $(h_n)_{n=1,2,...}$ with values in $\calF$ and for some $z\in(\Reals^+)^I$, define the sequence $(z^k)_{k=0,1,2,...}$ by $z^0=z$ and $z^k=h_k(z^{k-1})$ for $k\geq 1$. If the sequence $(h_n)_{n=1,2,...}$ visits every $f\in\calF$ infinitely often, then $z^k$ converges and the limit is independent of the sequence $h$, but may depend on $z$. In particular, the limit is a fixpoint of every $f\in \calF$.  }

% \anne{Yes, I think that the limit is a fixed point for every $f$. 
% If there is a unique fixed point (eg. for $f_1\circ \cdots f_n$), the result might not depend on the starting point). 
% But, (not really explicit above), is that it is not for all  $z\in (\Reals^+)^I$ in our case: we need it only for "valid" parameters, and request that they remain valid (ie above the fixed point). If we request this for all $z\in (\Reals^+)^I$, this is not applicable to our case. }

% \anne{Prove that the functions are concave (in the parameters and the latencies of the service curves, $\implies$ the  fixed point is unique (composition of concave and non-decreasing functions is concave)}











==> sot.tex <==


\section{Initial Phase: TFA Analysis} %\label{sec:initPhase}

%The analysis of a DRR system requires the computation of strict service curve for each node and each class of traffic, denoted $\beta = (\beta_i^v)_{1\leq i \leq n, v\in\mathcal{V}_i}$, as well as performing a FIFO analysis. In the previous section, we have seen that computing service curves requires the knowledge of the output burstiness bounds of each class, denoted $b^* = (b^{*, v}_i)$ (hence performing a FIFO analysis) and the computation of the output burstiness bounds of flows requires the knowledge of the service curves. Moreover, better service curves implies better burstiness bounds and conversely. 

%In addition,  PLP performs better than TFA for the per-class FIFO analysis and it is desirable to use PLP instead of TFA in the analysis. Executing the PLP analysis requires to the service curves the knowledge of per-node delays (with potential infinite values) and the decomposition of the network into a forest (by removing edges), and the output burstiness of each flow at each removed edge. 

Finally, many parameters are involved in the analysis of the system, that depend on each other. In order to accurately analyze the system, we propose a three-phase method: 

%\anne{For me it seems that the output burtiness is quite important for the DRR improvement. But (see other comment), is minimized by not having its "elementary operation" in the figure.}

\begin{table*}[htbp]
\centering
\caption{Operations}
\label{tab:cat}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l}
$\beta^v  = \drri_v\lp\alpha^v\rp$ & Compute a collection of service curves given a collection of input arrival curves $\alpha^v$ at node $v$.            \\ \hline\\
${\beta^v}' = \drrb_v \lp b^* ,\beta^v \rp$                              & Refines a collection of strict service curves  $\beta^v$ given a collection of output burstiness at node $v$,. \\\hline\\
$\lp d_i ,z_i\rp =\tfa_i \lp\beta_i\rp$  & TFA given service curves $\beta_i$ to compute per-node delay bounds $d_i $ and propagated burstiness $z_i$.            \\ \hline \\
$\zcuti = \plpcut_i \lp \beta_i, d_i\rp $ &
  Upper bounds the burstiness of flows of class $C_i$ at cuts. \\ \hline\\
$b^e = \plpb_{e,i} \lp \zcuti , \beta_i, d_i\rp$. &
  Upper bounds the aggregate burstiness flows of class $C_i$ carried by edge $e$.
\end{tabular}%
}
\end{table*}





Moreover, we want to use PLP as per-class network analysis as it provides better bounds compared to TFA. However, PLP requires per-node delay bounds computed by TFA;  Better per-node delay bounds improve the end-to-end bounds obtained by PLP. Note that PLP still applies without such per-node delay bounds but it might not perform as good. Moreover, PLP with per-node delay bounds of TFA performs better than TFA. Hence, our method starts with an initial phase where we compute bounds obtained by TFA. Specifically, in the initial phase, strict service curves and delay bounds are computed everywhere, as well as the burstiness of flows at cuts. Thus, at this point, PLP can compute an end-to-end delay bound for the flows of interest, given the initial bounds obtained by TFA. However, we can further improve these initial bounds by using PLP to compute better arrival curves and hence DRR strict service curves. Thus, we have a PLP refinement phase where we refine per-node strict service curve, per-node delay bounds, and   burstiness of flows at cuts. Lastly, we have a post-processing phase where use the obtained bounds inside PLP to compute and end-to-end bounds for the flows of interest. Therefore, our method for worst-case analysis of networks with DRR scheduling per-class can be divided into three main phases, illustrated in Fig.~\ref{fig:gen_method}:
\begin{enumerate}
    \item Initialization Phase (Section \ref{sec:initPhase}): We compute some valid per-node DRR strict service curves,  per-node delay bounds, and bounds on burstiness at cuts, i.e., $( \beta,d,\zcut )$; we use TFA per-class analysis and DRR strict service curves.
    \item Refinement Phase (Section \ref{sec:refinePhase}): We refine $( \beta,d,\zcut ) $; we use PLP per-class analysis and DRR strict service curves.
    \item Post-processing Phase (Section \ref{sec:postPhase}): Given $( \beta,d,\zcut )$, we compute end-to-end delay bounds; we use PLP.
\end{enumerate}
% \begin{itemize}
%     \item \textbf{Phase 0:} Compute some valid $\lp \beta,d,z \rp $ (i.e., per-node DRR strict service curves,  per-node delay bounds, and propagated burstiness), using existing method, i.e., Algorithm \ref{alg:tfa} in Section \ref{sec:tfa}.
%     \item \textbf{Phase 1:} Improve $\lp \beta,d,z \rp $, as much as possible, by means of refinements of Table \ref{tab:cat}, in an iterative way.
%     \item \textbf{Phase 2:} Given the improved $\lp \beta,d,z \rp $, use iPLP and compute an end-to-end delay bound for the flows of interest.
% \end{itemize}

In this section, we explain the initialization phase. In networks with cyclic dependencies, there is chicken-and-egg problem between DRR strict service curves and per-class network analysis TFA: On one hand, to compute DRR strict service curves we need to know arrival curves at inputs of every node. On the other hand, to compute the arrival curves at inputs of every node, we need to know DRR strict service curves at every node. To mitigate this dependencies, we compute a fixed-point: First, we apply TFA per-class network analysis given DRR strict service curves with no assumptions on arrival curves; this results in knowing arrival curves everywhere. Second, we improve  DRR strict service curves by taking into account these arrival curves. We then iterate between the TFA per-class network analysis and DRR strict service curves, until it converges. 

The method is summarized in \ref{alg:initPahse}: First, at lines 1-3, strict service curves of DRR in degraded operational mode (i.e., with no assumption on the interfering traffic) are computed at all nodes for all classes. Note that such curves only depend on the fixed parameters such as assigned quanta, the aggregate strict service curve, and maximum packet sizes of classes at a node (explained in Section \ref{sec:drrservice_dm}), and hence can be computed at this point. Second, at lines 5-7, one version of TFA (explained in Setion \ref{sec:tfa}) is applied for each class, given already computed service curves; hence, some bounds on propagated burstiness of flows $z$ and per-node delay bounds $d$ are computed. Third, at every node, at lines 9-11, an arrival curve at the input of a node is computed for every class, given the already computed propagated burstiness. Then, at line 12, DRR strict service curves are improved by taking into account these arrival curves. This procedure is then iteratively applied until we reach a fixed-point.

For the first time, at line 6, that per-class network analysis of TFA is applied, we might get finite bounds for some classes and infinite bounds  for other classes. But infinite bounds might become finite in the next iterations. This is because when improving DRR strict service curves (at line 12), the service curves of unstable per-class networks are improved thanks to the other stable per-class networks. Thus, it is possible that the next time per-class TFA is applied, it returns finite bounds with the improved strict service curves. We then iteratively apply this until for all classes with finite bounds, per-node delay bounds converges; it is guaranteed to converge. This is because for each per-node delay bound, a non-increasing sequence is obtained; as delay bounds are positive and the number of per-node delay bounds are finite it converges.  Note that computed  bounds are valid at each iteration, and we do not need to necessarily wait for convergence. At the end of this phase, we obtain some $( \beta,d,\zcut )$; values of $\zcut$ are extracted from $z$.

In this section, TFA is used as per-class network analysis, but as explained, PLP dominates TFA bounds as well as its stability region. In the next section, we explain the next phase, the PLP refinement phase, where we further refine the obtained bounds at this section using PLP. Note that at this point, an end-to-end delay bound for a flow of interest can be computed; it is equal to the sum of all per-node delay bounds in the path of the flow. However, as found numerically in Fig.~??, our method significantly improves the bounds obtained at this section. 




% 	\begin{algorithm}[htbp]
% 	\caption{Existing Algorithm for worst-case analysis  of networks with DRR}
% 	\begin{algorithmic}[1]
	
%     \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$}
%     	\State $\beta^v  \gets \drrnd_v $ 
%     \EndFor\\

% 	\While{$d$ is not converged}
% 		\For{each class $C_i$}
% 	    \State $\lp d_i ,z_i\rp \gets\tfa \lp\beta_i\rp$
% 	    \EndFor\\
	
% 	    \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$}
% 	    \State  Compute $\alpha^{\textrm{In}(v)}$ using $z^{\textrm{In}(v)}$.
%     	\State  $\beta^v \gets \drri_v \lp \alpha^{\textrm{In}(v)},\beta^v \rp$. 
%     \EndFor

% 	\EndWhile\\
		
% 	\end{algorithmic}
	


% 		\textbf{\\Output: }{$\lp d ,\beta, z\rp$: Per-node strict service curve, per-node delay bounds, and bounds on propagated burstiness of all flows for all classes\\}	
% 	\label{alg:tfa}
% \end{algorithm}

%	\begin{algorithm}[htbp]
	
 %   \SetKwInOut{Input}{Input}
%	\SetKwInOut{Output}{Output}
 %   \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$}{
  %  	 $\beta^v  \gets \betacdma$ \label{line:betaCDM}
%    }
 %   \BlankLine

%	\While{$d$ has not converged}{
%		\For{each class $C_i$}{
%	     $\lp d_i ,z_i\rp \gets\tfa_i \lp\beta_i\rp$ \label{line:tfa}
%	    }
%	\BlankLine
%	    \For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$}
%	    {
%	    \For{each class $C_i$}{
%	        Compute $\alpha^{v}_i$ from $z^{\textrm{In}(v)}_i$ \label{line:arrival}
%	       % $b_i^v \gets \sum_{e\in\textrm{In}(v)} \lp \sum z_i^e \rp $
	       % $\alpha^{v}_i \gets \sum_{e\in\textrm{In}(v)} \gamma_{r_f, b_i^v}$\;
%	        }
%    	$\beta^v \gets \drri_v \lp \alpha^{v}\rp$\;\label{line:drrService}
 %       }

%	}
		
%	\BlankLine

 %   \Output{$\lp d ,\beta, \zcut\rp$: Collection of per-node strict service curve, per-node delay bounds, and bounds on propagated burstiness of flows at cuts for all classes}
  %  \caption{Initial Phase: Initial Analysis with TFA}
%	\label{alg:initPahse}
%\end{algorithm}

% \section{Polynomial\anne{-size} Linear Programming (PLP): Background and Our Improvements} \label{sec:plp}
% \anne{I would rather avoid too many uses of the possessive form, especially in titles}

% \subsection{Background \cite{plp}}
%  Bouillard in \cite{plp} introduces a polynomial linear program (PLP) that computes end-to-end bounds in FIFO networks (i.e., per-class networks) for the flow of interest. To do so,
%  %PLP improves TFA bounds, and it also has a larger global stability region.
%  PLP considers an arrival time (resp. departure time) of a bit of interest of the flow of interest at the node this flow enters (resp. exits) the network. Then, it extracts some other times in between at other nodes. Thus, PLP considers finite set of times, where each of them is represented by a variable. Also, for each time variable at a node, two variables are introduced, denoting the cumulative arrival and departure functions for a flow at that node at that time. In other words, PLP extracts a finite set of times in the network as well as the cumulative functions of flows at those times. It then consists of writing network calculus relations as linear constraints in this finite set:
%  \begin{itemize}
%      \item Arrival curve constraints of each flow at its source
%      \item Service curve constraints at each node
%      \item Per-node delay bounds of TFA at each node 
%      \item Line Shaping Constraints at each node
%      \item FIFO constraints at each node
%      \item Monotonicity constraints
%  \end{itemize}
 
%   Then, a linear program maximize delay or backlog of the bit of interest. Every possible trajectory scenarios in the network is a feasible solution of PLP, as it satisfies the constraints; hence, the objective is an upper bound on worst-cases in the network. PLP requires a network to be a tree, otherwise some artificial cuts are introduced; PLP then can compute upper bounds on the burstiness of flows at cuts,  bounds on propagated burstiness  and end-to-end delay bounds of a single flow. 
  
%     PLP requires the strict curves to be piece-wise linear and convex, and arrival curves to be piece-wise linear and concave.
%   Also, as per-node delay bounds are part of the PLP constraints, it follows that the end-to-end delay bounds for a flows, obtained by PLP, is always smaller or equal to the sum of all per-node delay bounds in the path of the flow. Hence, PLP always improve the result of TFA. Also, it is observed that PLP gives larger stability region compared to TFA.
 
%   \subsection{Our Improvements}
%   Our first improvements is to use PLP to compute a bound on the propagated burstiness of aggregate of some flows in an intermediate node. Second, we presents iPLP, a PLP what supports non-convex strict service curves.
  
%   \subsubsection{Aggregate Output Arrival Curve}
%   PLP can compute an output arrival curve for an individual flow; then to compute an output arrival curve for an aggregate of some flows at a node, for example a DRR class, we need to aggregate the obtained output arrival curve for each flow. This might be pessimistic as we implicitly assume that the worst-case scenario for each flow can be achieved at the same time.  However, we want to use PLP and directly compute an output arrival curve for an aggregate of some flows. i.e., the worst-case scenario for the aggregate. We  use this improvements to compute output arrival curves for a DRR class at an intermediate node; a DRR class might contain several flows with different paths in the network, and this result enables us to directly compute output arrival curve for the class. 
  
%   \anne{$\mathbb{C}$ or $\mathscr{F}$? }Consider a system $\mathbb{S}$ and flows of interest that traverses $S$. Let $A_f \in \mathbb{C}$ (resp. $D_f \in \math{C}$) denote the cumulative arrival (resp. departure) of flow $f$, where $\mathbb{C}$ is the set of cumulative functions . Let $A = \sum_f A_f$ (resp. $D = \sum_f D_f$) denote arrival(resp. departure) of the aggregate of flows of interest. Assume the followings: A1) System $\mathbb{S}$ is causal. A2) The departure $D$ of system $\mathbb{S}$ is continuous. A3) Every flow of interest has a token-bucket arrival curve $\alpha_f $ with rate $r_f$ and burst $b_f$; also, $\alpha $  is the only constraints on the arrival of the flow of interest, i.e., every arrival $A_f  \in \mathbb{C} $ constrained by $\alpha_f$ is a possible arrival for this flow. A4) $\mathcal{B}$ is a backlogged bound for every possible arrival and departure of the aggregate of  flows of interest that belongs to system $\mathbb{S}$, i.e., $\forall (A,D) \in \mathbb{S}$, we have $A - D \leq \mathcal{B}$.
  
% \begin{theorem} \label{thm:backlog}
% 	Assume the assumptions A$1$-A$4$. Then, the departure of the aggregate of the flows of interest is constrained by  a token-bucket arrival curve with rate $r$ and burst $\mathcal{B}$ where $r = \sum_f r_f$, i.e., $\gamma_{r,\mathcal{B}}$.
% \end{theorem}

% The proof is given in Section \ref{sec:proof}. Note that in a specific case where we have only one flow of interest, assumptions A$1$-A$4$ are satisfied by those of Theorem 4 of \cite{plp}, and both Theorem  give exactly the same result.

% Theorem \ref{thm:backlog} enables us to use PLP and compute a bound on on the burstiness of the aggregate of some flows: We use the same PLP used to compute a backlog bound for a single flow yet the objective is now for the aggregate, i.e., a backlog bound for aggregate of flows in the network. Hence, by Theorem \ref{thm:backlog}, an output arrival curve an be computed for the aggregate.
%We will use this improvements to compute output arrival curves for a DRR class at an intermediate node; a DRR class might contain several flows with different path in the network, and above result enables us to directly compute output arrival curve for the class. 
%We denote this operation by $z_i^{\textrm{Out}(v)}  = \plpb_{v} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$: It computes a backlog bound for flows of class $i$ at the output of node $v$, using PLP with strict service curves $\beta_i$ and delay bounds $d_i$ of all nodes, and bounds on the burstiness of flows at cuts $z_i^ {E^{\scriptsize\textrm{cut}}_i}$.



%   \subsubsection{iPLP: a PLP that supports non-convex service curves}
%   PLP, as is, only supports piece-wise linear, convex strict service curves. However, authors in~\cite{drr_rtas,drr_ton} show that when delay bounds are small, non-convex strict service curves of DRR can be considerably beneficial. Specifically, we want to take into account $\beta^{\scriptsize\textrm{nc},v}$ as explained in Section \ref{sec:drrservice_dm} (see Fig. \ref{fig:ncService}).
  
  
% %  Specifically, if the service for a flow finishes in the first round (i.e., the first time that this class is visited by DRR scheduler). This motivate us to consider non-convex part of the DRR strict service curve only for the first service.
%  % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}


% \textbf{iPLP Construction:} Consider a node $v$ that offers $\beta^v$ a service curve that has two parts; a piece-wise linear convex and non-convex part, i.e., $\beta^v = \max \lp\beta^{\scriptsize\textrm{c},v},\beta^{\scriptsize\textrm{nc},v} \rp $; consider $\beta^{\scriptsize\textrm{nc},v}$ as shown in Fig.~\ref{fig:ncService}.  Construct iPLP  as follows: Define all variables and write all constraints exactly as PLP for delay bounds yet with one difference: At each node $v$, define $b_v \in \{0,1\}$ and add the following constraints:
% \begin{align}
%      D(t) - A(s) &\geq 0\\\label{eq:nc1}
%      D(t) - A(s) &\geq c_v(t-T_1) - Mb_v\\
%      D(t) - A(s) &\geq c_v(T_2-T_1) - M(1-b_v)\\
%      t - s &\leq T_2 + Mb_v\\
%      t - s &\geq T_2 - M(1-b_v)\label{eq:nc4}
% \end{align}
% where $M$ is a large positive integer.

% Then, we want to write the service curve constraint $\exists s, D(t) - A(s) \geq \beta^v(t-s) = \lp\beta^{\scriptsize\textrm{c},v}(t-s),\beta^{\scriptsize\textrm{nc},v}(t-s) \rp$ as linear constraints. Specifically, we want to write the non-convex part (i.e., $D(t) - A(s) \geq \beta^v(t-s) = \beta^{\scriptsize\textrm{nc}}(t-s)$ as linear constraints. Let $b^v \in \{0,1\}$ be a binary variable and $M$ be a large positive integer.
% \begin{align}
%      D(t) - A(s) &\geq 0\\\label{eq:nc1}
%      D(t) - A(s) &\geq c(t-T_1) - Mb^v\\
%      D(t) - A(s) &\geq c(T_2-T_1) - M(1-b^v)\\
%      t - s &\leq T_2 + Mb^v\\
%      t - s &\geq T_2 - M(1-b^v)\label{eq:nc4}
% \end{align}

% Let iPLP be built as follows: Define all variables and write all constraints exactly as PLP yet with one difference: At each node $v$, define$b^v \in \{0,1\}$ add constraints as in \eqref{eq:nc1}-\eqref{eq:nc4}.


% \begin{theorem}[iPLP: a PLP that supports non-convex service curves] \label{thm:iplp}
%     Consider iPLP as constructed above.  Then, 1) iPLP gives a valid delay bound for the flow of interest and 2) it improves the bound obtained with PLP.
% \end{theorem}

% The proof is in Section \ref{sec:proof}.



% \subsection{Summary and Notations of PLP Refinements}
% %   These operations  can be summarized with three functions as follows: 
%  \begin{itemize}
%      \item $z_i^{E^{\scriptsize\textrm{cut}}_i} = \plpcut_i \lp \beta_i, d_i\rp $: Computes  upper bounds on the burstiness of flows of class $C_i$ at cuts $E^{\scriptsize\textrm{cut}}_i$ using PLP given strict service curves $\beta_i$ and delay bounds $d_i$ of all nodes.
     
%      \item  $z_i^{\textrm{Out}(v)}  = \plpb_{v} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$: Compute a backlog bound for flows of class $i$ at the output of node $v$, using PLP given strict service curves $\beta_i$ and delay bounds $d_i$ of all nodes, and bounds on the burstiness of flows at cuts $z_i^ {E^{\scriptsize\textrm{cut}}_i}$.
     
%      \item $\dend_f = \iplpd_{f} \lp z_i^ {E^{\scriptsize\textrm{cut}}_i}, \beta_i, d_i\rp$ (resp. $\plpd_{f}$): Compute a end-to-end delay bound for flow $f$ of class $C_i$ using iPLP (resp. PLP) given strict service curves $\beta_i$ and delay bounds $d_i$ of all nodes, and bounds on the burstiness of flows at cuts $z_i^ {E^{\scriptsize\textrm{cut}}_i}$.
%  \end{itemize}
 




% \anne{Could we distinguish what we want to compute (the service curves and delay bounds) from how we compute it (precise implementation)? I guess at this point, any TFA++ algorithm would lead to the same result, and it might not be necessary to give the precise algorithm. Of course, in the implementation we have to choose the best one. (The bursts can be directly computed from the delays, if this is the part to add)}

% 	\begin{algorithm}[htbp]
% 	\caption{\textrm{SyncTFA}$\lp\mathcal{G}, \beta, \vec{r},  \vec{b}\rp$}
% 	\textbf{Inputs:}{
% 	$\mathcal{G}$: The graph induced by flows\\
% 	$\vec{r}$ and $\vec{b} $: rate and burst of flows\\
% 	$\beta$: Collection of offered strict service curves at all nodes\\
% 	}\\
% 	\begin{algorithmic}[1]
	
% 	\State $\forall$ edge $e \in \mathcal{E}^{\scriptsize\textrm{transit}}, z(e) \gets 0$
% 	\State $\forall$ node $v \in \mathcal{V}$, $d(v) \gets 0$
% 	\While{\textrm{True}} \Comment{\anne{Termination condition?}}
% 		\For{node $v$ $\leftarrow$ $1$ to $|\mathcal{V}|$ }
% 		        \State $d(v) \gets \mathcal{D}^{\scriptsize\textrm{NC}}\lp z\lp \textrm{In}(v)\rp,\beta(v)\rp$
% 		         \State $z\lp \textrm{Out}(v) \rp  \gets \mathcal{Z}^{\scriptsize\textrm{propagate}}\lp z \lp \textrm{In}(v) \rp,d(v)\rp $
% 	   %$\forall e \in \textrm{Out}(v),~
% 	   %\State \texttt{print}$\lp \vec{\dclass}(n) , \vec{\betaclass}(n) \rp$
% 		 \EndFor
% 	\EndWhile\\
		
% 	\end{algorithmic}
	


% 		\textbf{\\Output: }{$ \lp d\lp \mathcal{V} \rp,z\lp \mathcal{E}^{\scriptsize\textrm{transit}}\rp \rp$, a valid delay bounds at all nodes and  upper bounds on the propagated burstiness}	
% 	\label{alg:phase0}
% \end{algorithm}

% \subsection{PLP \cite{plp}}
% \anne{approximately same comment here: what do we need exactly to make the paper readable?}
% \hossein{TODO
% \begin{enumerate}
%     \item Background on PLP: PLP for delays, backlog, and the fixed point.
% \end{enumerate}}

% \subsubsection{Assumptions}
% \begin{enumerate}
%     \item A flow of interest \texttt{foi}
%     \item The graph induced by flows where the root is the last node traversed by \texttt{foi} is a tree. 
%     \item The scheduling policy is FIFO at all nodes. 
%     \item Token-bucket arrival curves for flows.
%     \item Convex, piece-wise linear strict service curves.
% \end{enumerate}

% \subsubsection{Overview and Definitions}
% PLP is a linear program that finds upper bounds on delays or backlogs for a flows or flows of interest. To do so, we consider a bit of interest of the flow of interest, and  we define two variables for this bit of interest: The time that it arrives at and departures the system. 

% % If we are interested to find a delay bound for this flows, we want to maximize the difference between these two time variables. Other variables and constraibnts
% As the graph induced by flows is a tree, it follows that each node $n$, except the root $N$, has a unique successor. We denote the successor of node $n$ by $\suc(n)$, and we let $\suc(N) = N + 1$. 

% Define $\depth$ as follows: Let $\depth(N+1) = 1$ and for every $n$, $\depth(n) = \depth\lp \suc\lp n \rp  \rp + 1$.

% Let $n^*$ be the first node that the flow of interest \texttt{foi} traverses, i.e., the first node of the path of. the flow of interest.


% \subsubsection{Variables}



% \subsubsection{Time Variables}
% Let $\tvar{N+1}{1}$ be the departure of the bit of interest. Then, for every node $n$, define  $\tvar{n}{k}$ with $k \in \{1, \ldots, \depth(n) \}$. The arrival time of the bit of interest is $\tvar{n^*}{1}$

% \subsubsection{Process Variables}
% For every node $n$ and every $f$ at $n$, define $\fvar{n}{f}{n}{k}$ with $k \in \{1, \ldots, \depth(n) \}$, where  $\fvar{n}{f}{n}{k}$ is a variable for the cumulative arrival function of flow $f$ at the input of node $n$ at time $\tvar{n}{k}$. 

% \subsubsection{Constraints}


% \begin{enumerate}
%     \item Time: $\forall$ node $n$
%         \begin{enumerate}
%             \item $\forall k \in \{1,\ldots,\depth(n)-1\}, \tvar{n}{k} \geq \tvar{n}{k+1}$
%             \item $\forall k \in \{1,\ldots,\depth(n)\}, \tvar{\scriptsize\suc(n) }{k} \geq \tvar{n}{k}$
%         \end{enumerate}
        
%     \item FIFO: $\forall$ node $n$ and $\forall k \in \{1,\ldots,\depth(\suc(n)) \}$,
%         \begin{enumerate}
%             \item $\forall$ flow $f \in \textrm{flows}(n).~\fvar{n}{f}{n}{k} == \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{k}$
%         \end{enumerate}
        
%     \item Service: $\forall$ node $n$,
%         \begin{enumerate}
%             \item $\sum_{f \in \textrm{flows}(n)}\lp \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{\scriptsize\depth(\suc(n))} - \fvar{n}{f}{n}{\scriptsize\depth(n)} \rp \geq 0$
%             \item $\sum_{f \in \textrm{flows}(n)}\lp \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{\scriptsize\depth(\suc(n))} - \fvar{n}{f}{n}{\scriptsize\depth(n)} \rp \geq R_n\lp \tvar{\scriptsize\suc(n)}{\scriptsize\depth(\suc(n))} - \tvar{n}{\scriptsize\depth(n)} - T_n \rp $
%         \end{enumerate}
        
%     \item TFA: $\forall$ node $n$ and $\forall k \in \{1,\ldots,\depth(\suc(n)) \}$ ,
%         \begin{enumerate}
%             \item $\tvar{\scriptsize \suc(n) }{k} - \tvar{n}{k} \leq d^{\scriptsize\textrm{TFA}}_n$
%         \end{enumerate}   
        
%     \item Arrivals:  $\forall$ flow $f$, let $n^{*}_f$ be the first node foe $f$, 
%         \begin{enumerate}
%             \item $\forall k < k' \in \{1,\ldots,\depth(n)\},~\fvar{n^{*}_f}{f}{n^{*}_f }{k} - \fvar{n^{\scriptsize\textrm{In}}_f}{f}{n^{*}_f }{k'} \leq b_f + r_f \lp\tvar{n^{*}_f }{k} -  \tvar{n^{*}_f }{k'}\rp $
%         \end{enumerate}    
%     \item Shaping:$\forall$ node $n$,  let $F^* = \textrm{flows}(n) \cap \textrm{flows}(\suc(n))$,
%         \begin{enumerate}
%             \item $\forall k < k' \in \{1,\ldots,\depth(n)\}$, $\sum_{f \in F^* } \lp \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{k} - \fvar{\scriptsize\suc(n)}{f}{\scriptsize\suc(n)}{k'}  \rp\leq \lmax + C_n\lp \tvar{\scriptsize\suc(n)}{k}  - \tvar{\scriptsize\suc(n)}{k'} \rp  $
%         \end{enumerate}       
        
%     \item Monotonicity: $\forall$ flow $f$, let $n^{*}_f$ be the first node foe $f$, ,
%         \begin{enumerate}
%             \item $\forall k \in \{1,\ldots,\depth(n^{*}_f)-1\}, \fvar{n^{*}_f}{f}{n^{*}_f}{k} \geq \fvar{n^{*}_f}{f}{n^{*}_f}{k+1}  $
%         \end{enumerate}    
        
%     \item Backlog: $\forall k  \in \{1,\ldots,\depth(n^*)\}$,
%       $ \fvar{n^{*}}{\scriptsize\texttt{foi}}{N+1}{1} -  \fvar{n^{*}}{\scriptsize\texttt{foi}}{n^{*}}{k} \leq b_{\scriptsize\texttt{foi}} + r_{\scriptsize\texttt{foi}} \lp \tvar{N+1}{1} - \tvar{n^{*}}{k}   \rp $
        
% \end{enumerate} 


% \subsubsection{Objectives}
%         \begin{enumerate}
%             \item Delay bound: $\max \lp \tvar{N+1}{1} - \tvar{n^*}{1}  \rp $
%             \item Backlog bound: $\max \lp \fvar{n^{*}}{\scriptsize\texttt{foi}}{N+1}{1}  - \fvar{N+1}{\scriptsize\texttt{foi}}{N+1}{1}  \rp $
%         \end{enumerate}




% Consider a system $\mathbb{S}$ and flows of interest that traverses $\mathbb{S}$. Let $A_f \in \mathbb{C}$ (resp. $D_f \in \mathbb{C}$) denote the cumulative arrival (resp. departure) of flow $f$, where $\mathbb{C}$ is the set of cumulative functions . Let $A = \sum_f A_f$ (resp. $D = \sum_f D_f$) denote arrival(resp. departure) of the aggregate of flows of interest. Assume
% \begin{description}
% 	\item [A1] System $\mathbb{S}$ is causal.
% 	\item [A2] The departure $D$ of system $\mathbb{S}$ is continuous.
% 	%, i.e., for $\forall A,D \in \mathbb{C}$, $(A,D) \in \mathbb{S}$, we have $A \leq D$ and 
% 	\item [A3] Every flow of interest has a token-bucket arrival curve $\alpha_f $ with rate $r_f$ and burst $b_f$; also, $\alpha $  is the only constraints on the arrival of the flow of interest, i.e., every arrival $A_f  \in \mathbb{C} $ constrained by $\alpha_f$ is a possible arrival for this flow. 
% 	\item [A4] $B$ is a backlogged bound for every possible arrival and departure of the aggregate of  flows of interest that belongs to system $\mathbb{S}$, i.e., $\forall (A,D) \in \mathbb{S}$, we have $A - D \leq B$.
% 	\item
% \end{description}

% \begin{theorem} \label{thm:backlog}
% 	Assume the assumptions A$1$-A$4$. Then, the departure of the aggregate of the flows of interest is constrained by  a token-bucket arrival curve with rate $\sum_f r_f$ and burst $B$.
% \end{theorem}

% Note that in a specific case where we have only one flow of interest,Theorem \ref{thm:backlog} gives exactly the same result as \cite[Theorem 4]{PLP}.



% \hossein{TODO
% \begin{enumerate}
%     \item Background on PLP: PLP for delays, backlog, and the fixed point.
%     \item Theorem for binary variable for DRR strict service Curves
%     \item Theorem for binary variable for stair arrival curves, (?) could be skipped for this paper
% \end{enumerate}}





